Rumor Source Detection under Querying with Untruthful Answers

Social networks are the major routes for most individuals to exchange their opinions about new products, social trends and political issues via their interactions. It is often of significant importance to figure out who initially diffuses the information, ie, finding a rumor source or a trend setter. It is known that such a task is highly challenging and the source detection probability cannot be beyond 31 percent for regular trees, if we just estimate the source from a given diffusion snapshot. In practice, finding the source often entails the process of querying that asks "Are you the rumor source?" or "Who tells you the rumor?" that would increase the chance of detecting the source. In this paper, we consider two kinds of querying: (a) simple batch querying and (b) interactive querying with direction under the assumption that queries can be untruthful with some probability. We propose estimation algorithms for those queries, and quantify their detection performance and the amount of extra budget due to untruthfulness, analytically showing that querying significantly improves the detection performance. We perform extensive simulations to validate our theoretical findings over synthetic and real-world social network topologies.

==> background_yy.tex <==
\section{Model and Preliminaries}
\label{sec:model}

\subsection{Model}
%diffusion process, blah, blah.. standard things...
\noindent{\bf \em Rumor diffusion.} We describe the rumor spreading
model which is commonly adopted in other related work, e.g.,
\cite{shah2010,shah2012,zhu2013}.  We consider an undirected graph
$G=(V,E),$ where $V$ is a countably infinite set of nodes and $E$ is
the set of edges of the form $(i,j)$ for $i, j\in V$.  Each node
represents an individual in human social networks or a computer host
in the Internet, and each edge corresponds to a social relationship
between two individuals or a physical connection between two Internet
hosts.  We assume a countably infinite set of nodes for avoiding the
boundary effects. As a rumor spreading model, we consider a SI model,
where each node is in either of two states: {\em susceptible} or {\em
  infected}. All nodes are initialized to be susceptible except the
rumor source, and once a node $i$ has a rumor, it is able to spread
the rumor to another node $j$ if and only if there is an edge between
them.  Let a random variable $\tau_{ij}$ be the time it takes for node
$j$ to receive the rumor from node $i$ if $i$ has the rumor. We assume
the $\tau_{ij}$ are exponentially distributed with rate $\lambda>0$
independently with everything else. Without loss of generality, we
assume that $\lambda=1$. We denote $v_1 \in V$ by the rumor source, which
acts as a node that initiates diffusion and denote $V_N \subset V$ of $N$ infected
nodes under the observed snapshot $G_N\subset G$. In this paper, we consider 
the case when $G$ is a regular tree
and our interest is when $N$is large, as done in many prior work
\cite{shah2010,shah2012,Khim14,dong2013,Zhang2014}.

% but our analytic results on
% trees in Sections~\ref{sec:noninteractive} and Section
% \ref{sec:interactive} can be used for designing a practical rumor
% source estimator even for loopy graphs as described in Section
% \ref{sec:numerical}.



\begin{comment}
  For general loopy graphs, the rumor source detection problem is not
  easy to analyze, and most properties derived in the tree graphs do
  not extend, e.g., the ML estimator is NP-hard to compute.  However,
  following the implications from the results in regular trees, one
  can design a heuristic algorithm that performs well for general
  graphs.  For example, in \cite{shah2010tit}, they suggest to choose
  BFS (Breadth First Search) first, and use the rumor centrality of
  the tree as the rumor source estimator for the general graph.
\end{comment}

% then, the object of this paper is finding the correct rumor source
% detection probabilities by using proper queries. In this model, we
% consider the rumor infection as a SI model.  For the rumor
% propagation model, let's consider that once a node $i$ has a rumor,
% it is able to spread it to another node $j$ if and only if there is
% an edge between them ($(i,j)\in E$). Let $\tau_{ij}$ be the time it
% takes for node $j$ to receive the rumor from node $i$ once $i$ has
% the rumor. We assume the $\tau_{ij}$ are independent and have
% exponential distribution with rate $\lambda>0$. Without loss of
% generality, we assume that $\lambda=1$.

%To achieve our goal, we propose two intuitive querying algorithms for
%non-interactive and interactive queries, respectively.

%In the next section, we first provide the preliminaries in absence of
%querying, required to develop our querying algorithms and understand
%the amount of room for improvement via querying.

\begin{comment}
of the estimator by introducing the concept of \emph{querying}. We
consider two kinds of querying which are interactive and
non-interactive querying.  Interactive querying scenario assumes that
we can obtain additional information with each single query. Then we
can utilize those additional information to determine the next
estimator and iterate queries.  However, non-interactive querying
scenario involves simultaneous querying without interactive
question-and-answer mechanism. In non-interactive case we cannot
obtain additional information from each query.

The notion of \emph{querying budget} will be used throughout this
paper.  We say there are $K$ querying budgets when we have $K$ chances
of question-and-answering in interactive querying scenario or we have
$K$ amount of nodes that can be simultaneously picked in
non-interactive querying scenario. We will closely investigate each
querying scenario and derive the lower-bound guarantee of improved
detection probability with given amount of $K$ querying budgets.



So far we discussed about the performance of ML estimator for
detecting rumor sources. However, the detection probability was quite
low; less than 1/2 in every case.  In practical situations, we do not
usually determine various properties of a stochastic process in a
single guess. Rumor source detection is a part of these estimation
processes, and we can think about doing simultaneous/sequential
multiple guesses instead of doing a single guess in order to improve
the credibility of the estimation.

We aim at improving detection probability of the estimator by
introducing the concept of \emph{querying}. We consider two kinds of
querying which are interactive and non-interactive querying.
Interactive querying scenario assumes that we can obtain additional
information with each single query. Then we can utilize those
additional information to determine the next estimator and iterate
queries.  However, non-interactive querying scenario involves
simultaneous querying without interactive question-and-answer
mechanism. In non-interactive case we cannot obtain additional
information from each query.

The notion of \emph{querying budget} will be used throughout this
paper.  We say there are $K$ querying budgets when we have $K$ chances
of question-and-answering in interactive querying scenario or we have
$K$ amount of nodes that can be simultaneously picked in
non-interactive querying scenario. We will closely investigate each
querying scenario and derive the lower-bound guarantee of improved
detection probability with given amount of $K$ querying budgets.
\end{comment}

\begin{figure}
\begin{center}
\subfigure[A simple batch querying.
]{\includegraphics[width=0.24\textwidth]{figs/Noninter}\label{fig:Noninter}}
\hspace{-0.2cm} \subfigure[Interactive querying with direction.
]{\includegraphics[width=0.24\textwidth]{figs/Inter}\label{fig:Inter}}
\hspace{0cm}
 \end{center}
\caption{Examples of two querying types with untruthful
  feedbacks. In (a), the querier selects a candidate set (a dotted
  circle) and asks just one question (i.e., $r=1)$ in a batch. In (b),
  starting from the initial node, the querier first asks ``Are you the
  rumour source?'', and if no, she further asks ``Who spreads the rumor to
  you?'', where the querier interactively tracks the true source, but the
  queriees may be untruthful (RS: Rumor Source). }
\label{fig:querying}
% \vspace{-0.5cm}
\end{figure}




%\begin{figure}
%\centerline{\includegraphics[width=0.3\textwidth]{figs/Noninter}} \caption{Explanation
%of $T^v_u$. $T^1_2$ is 3 because there are 3 nodes in the subtree
%rooted at node 2 considered node 1 is the overall root of the
%tree.}  \label{fig:subtree} \end{figure}

% \subsection{Querying Scenario}

\smallskip
\noindent{\bf \em Querying with untruthful answers.}  A detector is
allowed to query the nodes, where querying refers to a process of
asking some questions (which will be shortly clarified depending on
the querying scenarios).  The detector is given some querying budget
$K,$ where we assume that one budget is used to ask one question.  In
this paper, we consider two types of queries (see
Fig.~\ref{fig:querying}), where a queriee may be untruthful, as
modeled in what follows:


% of a particular node whether she is a rumor source or not, where we
% assume that the queriee is truthful in answering questions. It is
% clear that more queries would help to detect the rumor source and
% the main goal in this paper is to quantify its effect. We consider
% the following two querying scenarios.


%  with a given budget $K,$ where a unit budget is used to ask a unit
% of questions.

% % Depending on how querying is performed, we consider the following two
% % querying scenarios:

\smallskip
\begin{compactenum}[$\circ$]
\item {\bf \em Simple batch querying.}  This query is parameterized by
  $r$, where a querier first chooses $K/r$  ($K$ is a multiple of $r$ for expositional convenience)
  candidate nodes to each of which an {\em identity question} of ``Are
  you the rumour source?'' is asked $r$ times. We call $r$ the
  {\em repetition count} throughout this paper.
  Each queriee $v$ is
  truthful in answering each question only with probability $p_v,$ i.e.,
  even if she is the rumour source, she lies with probability $1-p_v.$
  We assume that the answers are independent over the $r$ queries across
  the queriees. We assume the homogeneous case when $p_v = p$ for all
  $v \in V_N,$ and $p > 1/2,$ i.e., all users are biased with truthful
  answers. For example, Fig~\ref{fig:Noninter} shows a
  candidate set of nodes insides a dotted circle, where with $r=1$ we
  have four ``yes'' nodes and five ``no'' nodes.


\smallskip
\item {\bf \em Interactive querying with direction.}  In this querying
  type, there are two questions, where one is the identity question, as
  in the simple batch querying and another is the {\em direction
    question} of ``From whom you have heard the rumor?.''  This query is
  also parameterized also by $r,$ where the querying process occurs in
  the following interactive manner: A querier first chooses an initial
  node to ask the identity question, and further asks the direction
  question $r$ times (i.e., repetition count), if the queriee answers
  that she is not the rumor source, but the querying process stops when
  the queriee says that she is the rumor source or the entire budget $K$
  is exhausted. A querier determines the next queriee from $r$
  questions, where each queriee $v$ is truthful for the identity
  question, but she is truthful for the direction question only with
  probability $q_v.$\footnote{In this type of query, we model
    untruthfulness only in the direction question, because we aim at
    purely focusing on the impact of untruthfulness in the interactive
    search of the true rumour source, which seems to be the critical
    component in this type of querying.} In other words, she lies for
  the direction question with probability $1-q_v$ and designates a node
  uniformly at random out of all neighbors except for the node who truly
  spreads the rumor to $v$ as a bogus ``parent''. Then, the querier 
  chooses one of neighbor node as parent of $v$ and repeats the same procedure.
  As in the simple batch
  querying, we assume the homogeneity in truthfulness that $q=q_v$ for
  all $v \in V_N,$ and $q > 1/d,$ i.e., users' bias for truthful
  answers\footnote{In $d$-regular trees, when $q=1/d$, the answer for
    the direction question turns out to be uniformly random.}
  Fig~\ref{fig:Inter} shows an example scenario that starting from the
  initial node, a sequence of nodes answer the interactive queries
  truthfully or untruthfully.



% ----------------------- If the node reveals itself is not the rumor
%   source then ask \emph{additional} queries as ``From whom you have
%   heard the rumor?'' which is an {\em direction question}, $r$
%   times.  Each queriee $v$ is truthful in answering for the identity
%   question and is truthful in answering for the direction question
%   with probability $q_v,$ i.e., she lies with probability $1-q_v$
%   for saying its parent node \footnote{For simplifying the analysis,
%   we assume that the queried node answer the truth for the identity
%   question in the interactive querying scenario.}.  We also assume
%   that the answers of direction questions are independent across the
%   $r$ queries. In this setting, a querier chooses the queriee
%   iteratively, where who will be the $k$-th queriee may be
%   determined by the answer of $(k-1)$-th queriee.


\end{compactenum}

% In practice, the queried node may not give the correct answer for
% the questions so that we need to consider the scenarios that the
% feedback of all queries are not true \ie some of them has a noise
% with their answer.  In this paper, we consider the following
% feedback scenario.  \smallskip \begin{compactitem}[$\circ$] \item
% {\bf Feedback scenario.} When an infected node $v$ is selected by a
% querier, the node reveals the correct answer with probability
% $p_v>0$ for the first question (Are you the rumor source ?) in the
% non-interactive scenario. For the interactive case, the node reveals
% the correct answer for the first question but reveals the correct
% answer with probability $q_v >0$ for the second question (From whom
% you have heard the rumor ?), respectively\footnote{In our work, we
% do not consider the noisy feedback for the first question in the
% interactive scenario for simple analysis.}.  Thus, the rumor source
% detection without queries in most prior works corresponds to the
% case when $K=1$ and $p_v=1$ for all $v\in V_N$.


\smallskip
\noindent{\bf \em Goal.} Our goal is to propose the efficient estimation
algorithms for both types of queries with users' untruthfulness that are
practically implementable. Especially, we aim at theoretically
quantifying the detection performance of our proposed algorithms by
providing the lower bound of the required budget $K$ to satisfy any
arbitrary detection probability, i.e., the sufficient budget $K$ for the
target detection quality.


% The goal of this paper is to quantitatively
% understanding how much querying helps in improving the detection
% probability for both querying scenarios with unfaithful answers.
% To do this, designing simple and smart algorithms is a challenging
% issue to guarantee the high source detection performance. In the
% following sections, we introduce the source estimation algorithm
% for both querying scenarios to resolve these issues. Before seeing
% this, we remind a preliminary result which is used in our algorithms.
\vspace{-0.2cm}
\subsection{Preliminaries: Rumor Centrality}
\label{sec:rumor_center}

As a preliminary, we explain the notion of {\em rumor centrality,} which is a
graph-theoretic score metric and is originally used in detecting the
rumor source in absence of querying and users' untruthfulness, see
\cite{shah2010}. This notion is also importantly used in our framework
as a sub-component of the algorithms for simple batch querying and
interactive querying with direction.
% In this section, we provide the known results for rumor source
% detection in absence of querying, i.e., $K=1$.  One of the most
% popular estimators is based on maximum likelihood (ML).
In regular tree graphs, Shah and Zaman \cite{shah2010} showed that the
source chosen by the Maximum Likelihood Estimator (MLE) becomes the node
with hightest rumor centrality. Formally, the estimator chooses $v_{RC}$ as
a rumor source defined as
\begin{eqnarray}\label{eqn:ML}
v_{RC} &=& \arg\max_{v \in V_N} \mathbb{P}(G_N | v=v_1)\cr
       &=&\arg\max_{v \in V_N} R(v, G_N),
\end{eqnarray}
where $v_{RC}$ is called \emph{rumor center} and $R(v, G_N)$ is the
rumor centrality of node $v$ in $V_N$. The rumor centrality of a
particular node is calculated only by understanding the graphical
structure of the rumor spreading snapshot, i.e., $R(v, G_N) =N!
\prod_{u \in V_N} (1/T^v_u)$ where $T^v_u$ denotes the number of nodes
in the subtree rooted at node $u$, assuming $v$ is the root of tree
$G_N$ (see \cite{shah2010} for details).
% \footnote{Refer \cite{shah2010} to see the details about the rumor
% centrality in the $d$-regular tree.}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> interactive_jy.tex <==

\section{Interactive Querying with Detection}
\label{sec:interactive}
\subsection{Algorithm based on ML for next node selection}
A source finding algorithm for interactive queries consists of the
following steps: We first need to appropriately choose the repetition
count $r$ and the initial node $v_I$ to ask the identity question.
If she is not the source then ask the direction questions $r$ times. 
From the answers of querying, the querier chooses a next node to perform 
the same procedure. Hence, the next queried node is determined by the previous
queried node when the initial node is $v_I$. Let $\mathcal{P}(v_I)$ be a 
policy that chooses the next queried 
node and let $V^r =\{v^1, v^2, \ldots, v^{K/r}\}$ be the set of queried nodes by next
node selection policy $\mathcal{P}.$ Then, we will be given an instance of the direction
answers, which we denote by a vector
$D_{r}^{i} = D_{r}(q)=[y_1, y_2, \ldots, y_{d}]$ with $0\leq y_j \leq d$ that
represents the number of ``indications'' answers of the $j$-th neighbor 
node by the queried node $v^i$. Let $pa(v)$ be the true parent of a node $v \in V_N$
and let $nb(v)$ be the set of all neighbors of $v$. 
Then, the next queried node is selected by some ML from the data
$D_{r}^{i}$ and repeat same procedure as in the first step. 
Then, to maximize the detection performance, that solves the following optimization:
\vspace{-0.3cm}
\separator
\vspace{-0.4cm}
\begin{align}\label{eqn:OPT1}
% \displaystyle
\text{\bf OPT-I:} &  \quad \max_{1\leq r \leq K} \max_{\mathcal{P}(v_I)}
\left(\prod _{i=1}^{K/r}\max_{v \in nb(v^i)}\bprob{G_N,D_{r}^{i}| v=pa(v^i)}\right),
\end{align}
where the most inner max corresponds to the ML estimator given the
diffusion snapshot $G_N$ and the query answer snapshot $D_{r}^{i}$
which are independent to $1\leq i \leq K/r$.
\vspace{-0.3cm}
\separator

\smallskip
\noindent{\bf \em Challenges.} We now explain the technical challenges
in solving {\bf OPT-I}. To that end, let us
consider the following sub-optimization in {\bf OPT-I} for a fixed $ 1\le
r \le K$:
\begin{align}\label{eqn:subOPT1}
% \displaystyle
\text{\bf SUB-OPT-I:} &  \quad \max_{\mathcal{P}(v_I)}
 \left(\prod _{i=1}^{K/r}  \max_{v \in nb(v^i)}\bprob{G_N,D_{r}^{i}| v=pa(v^i)}\right).
\end{align}
To solve {\bf SUB-OPT-I}, let $\bprob{G_N, \mathcal{D}_r|V^r}$ be the probability
in the parentheses of \eqref{eqn:subOPT1} then 
\begin{align}
  \label{eq:tra}
\max_{\mathcal{P}(v_I)}
& \bprob{G_N, \mathcal{D}_r|V^r}\cr
& =\max_{\mathcal{P}(v_I)}\left(\bprob{v_1 \in V^r }\times \bprob{G_N, \mathcal{D}_r|V^r, v_1 \in V^r}\right)\cr
& =\underbrace{\max_{\mathcal{P}(v_I)}\bprob{v_1 \in V^r }}_{(a)}\times 
\underbrace{\max_{\mathcal{P}(v_I)}\bprob{G_N, \mathcal{D}_r|V^r, v_1 \in V^r}}_{(b)},\cr
\end{align}
where we will discuss the analytical challenges in $(a)$ and $(b),$
respectively.
First, the term $(a)$ is difficult to analyze, because
it is not easy to obtain the optimal policy $\mathcal{P}(v_I)$
because the number of candidate sets may be very large to handle. 
Second, to see the challenging in $(b)$,
let $D_{r}^{i}=[x_1, x_2,\ldots, x_{d}]$ be the vector where
$0 \leq x_i\leq r$ is the number of indications by the queried node as
the parent node. Then, we can also
obtain the MLE for the parent of $v^i$ as
\begin{equation}\label{eqn:MAP2}
\begin{aligned}
\hat{v}_{\tt ml}^{i+1}&=\arg\max_{v \in nb(v^i)}\bprob{G_N,
D_{r}^{i}|v=pa(v^i)}\\ &\stackrel{(a)}{=}\arg\max_{v \in
  nb(v^i)}\bprob{G_N,|v=pa(v^i)}\bprob{D_{r}^{i}|v=pa(v^i)}.\\
\end{aligned}
\end{equation}
In this case, the first term in \eqref{eqn:MAP2} is given
by $\prob{G_N,|v=pa(v^i)}=\sum_{u \in T_v}R(u,G_N)$ where $T_v$
is the subtree rooted at node $v$ because if $v$ is the parent of
$v^i$ then one of node in $T_v$ is the rumor source. the second 
term is Multinomial distribution that $pa(v^i)$ has the probability 
$q$ and $(1-q)/(d-1)$, for other neighbor nodes of $v^i$.
However, it is not easy to characterize this probability and obtaining the second
probability in \eqref{eqn:MAP2} for every queried node $v^i$.


Motivated by this, we propose an algorithm producing an
approximate solution of {\bf OPT-I}. The key of our approximate algorithm
is to choose $V^r$ that allows us to analytical compute the detection
probability for a given $r$ so as to compute $r$ easily, yet its
performance is close to that of {\bf OPT-I}.
\subsection{Algorithm based on Parent node and Majority Rule}

\begin{algorithm}[t!]
 \KwIn{Rumor set $V_N$, querying budget $K$, degree $d$, and truth
   probabilities $q>1/d$} \KwOut{Estimated rumor source $\hat{v}$}
 Calculate the rumor centrality $R(v, G_N)$ for all $v \in G_N$ as in
\cite{shah2010} and let $ s \leftarrow \arg\max_{v \in V_N} R(v, G_N)$\;
 $r \leftarrow \left\lfloor1+\frac{2d(1-q)^2 \log\log
   K}{3(d-1)}\right\rfloor$\; \While{}{ \eIf{$s = v_1$} { Return $s$\;
     $K \leftarrow K-1$\; } {\If{$K\geq r$} {Count the number of
       ``indication'' (i.e., She has spread the rumor to me) for the
       direction question among $nb(s)$, and choose the largest
       counted node with a random tie breaking \; Denotes the selected
       node by $s$\; $K \leftarrow K-r$\; } } { Return $s$\;} } Return
 $\hat{v}=s$\;
 % \caption{RCP (RC-based Parent tracking) Algorithm \note{change the
 %     format following Algorithm 1.}}
 \caption{Estimation for Interactive Querying with Direction}
\label{alg:interactive}
\end{algorithm}

We now propose an algorithm that overcomes the afore-mentioned
challenges in $(a)$ and $(b)$ in \eqref{eq:trade}. The key idea is that
for $(a)$ we adopt a {\em  parent selection} as the next queried node
and for $(b)$ we simply apply a {\em majority-based rule}, as
will be clarified soon.

We first formally describe our algorithm in {\bf
  Algorithm~\ref{alg:interactive}} and explain how it operates,
followed by presenting the rationale behind it: we first calculate the
rumor centrality of all nodes in $G_N$ (Line 1), where $s$ is set to be
the rumor center. Then, we appropriately choose the repetition count as
in Line 3, and query the identity question to the rumor center $s$ (Lines 4-6).
If she is not the source then ask the direction questions $r$ times, and count the
number of ``indications'' for its neighbor (Line 9). Then, it chooses the largest 
counted node with a random tie breaking and repeat the same procedure (Line 12).
The algorithm stop when there is a node which reveals itself as the rumor 
source within $K$ queries, otherwise, it output the last queried node as 
the estimator.

\smallskip
\noindent{\bf \em Rationale.} We now provide the rationale of {\bf
  Algorithm~\ref{alg:interactive}} from the perspective of how we handle the
analytical challenges in \eqref{eq:trade}  so as to approximately solve
{\bf OPT-I} in an approximate manner.

\smallskip
\begin{itemize}
\item[$\circ$] {\em Selection of initial node and Parent as the next queried node:} 
From the fact that the rumor source is nearby the rumor center with high probability, 
we see that the best 
strategy for selecting the initial node to query is selecting the rumor center. Furthermore,
even though there is untruthful answer of queries, selecting the parent as the next queried 
node is quite good from the same reason. 


\item[$\circ$] {\em  Majority rule 
    to select the parent:} Instead of using the exact calculation of MLE in \eqref{eqn:subOPT},
  because \note{...}
\end{itemize}

Using the above approximation techniques, we are able to have the closed
and approximate form of {\bf SUB-OPT-I}, which allows us to compute the
best $r^\star$ that maximizes the detection probability as in
$r^*= \left\lfloor1+\frac{2d(1-q)^2 \log\log K}{3(d-1)}\right\rfloor.$



%\smallskip
%\noindent{\bf \em (a) Choice of the initial node $v_I$ and $r$:} In
%the interactive scheme, the choice of initial queried node is very
%important for a given budget $K$. However, without any priori
%information about the source, MLE (rumor center) may be best candidate
%node as the initial queried node. Hence, in the first part (line 1 -
%2), similar to the previous algorithm, it calculates the rumor
%centrality $R(v,G_N)$ by using given snapshot $G_N$, and selects the
%maximum centrality node $s$. Then the querier ask the identity
%question to this node. If the node answer ``yes" then the algorithm
%stop and output the estimated node as this node.  If this node does
%not reveals itself as the rumor source then, ask additional direction
%question and the node reveals the true parent node with probability
%$q$, which means that the queried node $s$ reveals its parent $pa(s)$ with
%probability $q$ and the other node $u \in nb(s)$ with probability
%$(1-q)/(d-1)$. Similar to the batch querying scenario, the right value
%of the query repetition count $r$ is of critical importance in
%achieving high detection probability, where $r$ trade offs the radius
%for searching and the quality of the selected queriees. For example,
%when $r=1,$ then we can query to large number of nodes, but only one
%query can be asked for each node, in which case, there exists a
%possibility that the distance between the source and next queried node
%increases due to the answer of wrong direction.  From this fact, we
%also analytically study and derive the ``optimal'' value of $r=
%\left\lfloor1+\frac{2d(1-q)^2 \log\log K}{3(d-1)}\right\rfloor$ that
%minimizes the error probability under our framework, which is thus
%used in our algorithm.
%
%\smallskip
%\noindent{\bf \em (b) Filtering and searching the source.}  The
%querier now gives queries to each selected infected nodes for $r+1$
%times. From the fact that each queried node answer the truth with
%probability $q$ for the direction answer at each time, the algorithm
%cumulates the number of reveals who the parent node is. In the line 9,
%the algorithm chooses the node which has the maximum counted of
%indication among the neighbors $nb(s)$ of the queried node $s$ with a
%random tie breaking rule. Then, the querier chooses this node and
%repeat this query procedure (line 5-13). If the querier chooses the
%source within $K$ queries then the algorithm stop and otherwise, it
%output the last queried node as the estimator.




\subsection{Detection Performance}
We now provide analytical results on the detection performance of {\bf
  Algorithm~\ref{alg:interactive}}. We first start by the result that presents the lower
bound of the detection probability for a given repetition count $r$ in
Proposition~\ref{prop:inter_prob} Then, in
Theorem~\ref{thm:interactive}, we present the lower bound on the
budget for any given detection probability $0< 1-\delta<1.$

\begin{proposition}
  \label{prop:inter_prob}
  For $d$-regular trees ($d\geq 3$), the detection probability of the
  Interactive Querying with Direction for given $K,$ $q > 1/d$ and $r$ is
  lower-bounded by:
\begin{align}
  \label{eqn:detect2}
  \bprob{\hat{v}=v_1}\geq 1-ce^{-2 g_d (r,q)^3
  \left(\frac{K}{r+1}\right)\log \left(\frac{K}{r+1}\right)},
\end{align}
where $g_d (r,q):= 1- e^{-\frac{r(d-1)}{3d(1-q)}}$ and
$c=(8d+1)/d$.
\end{proposition}
\smallskip
This result implies that the error probability of detecting the source decaying 
exponentially with respect to $K$ for a given $r$. Furthermore, we see that there 
is a tradeoff for selecting $r$ to maximize the probability in \eqref{eqn:detect2}. 
From this result, we obtain the
best $r*$ which maximizes the probability in \eqref{eqn:detect} and we have the following
theorem.

\smallskip
\begin{theorem}
\label{thm:interactive}
For any given sufficiently small $\delta>0,$ the detection probability for $d$-regular
tree is at least $1-\delta,$ if
\begin{align}
\label{eqn:elower1}
    K\geq \frac{(2d-3)/d(\log(7/\delta))}{q^3\log \Big(\log (7/\delta)\Big)}.
    \end{align}
\end{theorem}

\smallskip
This result implies that if there is untruthful answer of direction
with probability $q>1/d$ for the interactive query then it requires
$1/q^3$ times more budget compared to the case without lying to
guarantee the target detection probability. Furthermore, if $q\simeq
1/2$ then, it requires about 8 times more budget for $d$-regular
tree. Furthermore, if $q=0.4$ then it needs $K\geq 51$ to achieve 
the detection probability at least 95\% for $d=3$. 
Therefore, it requires much less queries than that of batch
querying which reducing the order of $1/\delta$ to $\log (1/\delta)$
because the answer of direction gives the path information of the
rumor source from the queried node whereas the batch querying consider
all nodes regardless of the path.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> lemma.tex <==
\section{Proof of Lemmas}
\label{sec:lemma}

























%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> noninteractive.tex <==

\section{Detection Using Simple Batch Queries}
\label{sec:noninteractive}

\subsection{Algorithm based on MLE and Rumor Centrality}

A source estimation algorithm for simple batch queries consists of the
following steps: We first need to appropriately choose the repetition
count $r$ and the candidate set $C_r \subset V_N$ of size $K/r$ and ask the queries
to the nodes in $C_r.$ Then, we will be given an instance of the
answers, which we denote by a vector
$A_r = A_{r}(p)=[x_1, x_2, \ldots, x_{K/r}]$ with $0\leq x_i \leq r$ that
represents the number of ``yes'' answers of the $i$-th node of $C_r.$

Then, it is natural to consider an algorithm based on ML, to maximize
the detection performance, that solves the following optimization:
\separator
\vspace{-0.2cm}
\begin{align}\label{eqn:OPT}
% \displaystyle
\text{\bf OPT:} &  \quad \max_{1\leq r \leq K} \max_{C_r}
  \max_{v \in C_r} \bprob{G_N,A_{r}| v=v_1},
\end{align}
where the most inner max corresponds to the ML estimator given the
diffusion snapshot $G_N$ and the query answer snapshot $A_r.$
\vspace{-0.2cm}
\separator

\begin{comment}
Note that
\begin{align}\label{eqn:MAP}
\hat{v}_{\tt ml}&=\arg\ \max_{v \in C_r} \bprob{v=v_1|G_N,A_{r}}\\
&\stackrel{(a)}{=}\arg\max_{v \in
  C_r}\bprob{G_N|v=v_1}\bprob{A_{r}|v=v_1},
\end{align}
where $(a)$ is from the fact that $G_N$ and $A_{r}$ are independent.
\end{comment}
% \begin{align}\label{eqn:OPT}
%  \underset{1\leq r \leq K}{\max} \underset{C_r}{\max}
%   \biggl(\underset{estimator }{\max} \mathbb{P}(\hat{v}=v_1|G_N,K^{r}_{p}) \biggl)
% % & \text{subject to}   & & \text{\# ~of~ budget} \leq K,
% \end{align}
% Before designing the batch querying algorithm, we first consider an
% optimization problem which maximizes the detection probability for
% given $K, r,$ and $p>1/2$ \footnote{We consider the case $p>1/2$
%   because if $p<1/2$, then it is same by setting the case that all
%   queried nodes answer the truth with probability $1-p$ and if $p=1/2$
%   then there is no information gain by the queries}. To do this, let
% $\hat{v}$ be the estimator of an algorithm then our object is to solve
% the following optimization problem:
% \begin{equation}\label{eqn:OPT}
% \begin{aligned}
% & \underset{1\leq r \leq K}{\text{max}} \underset{V^r}{\text{max}}
%   \biggl(\underset{estimator }{\text{max}} & &
%   \mathbb{P}(\hat{v}=v_1|G_N,K^{r}_{p})\biggl)\\ & \text{subject to}
%   & & \text{\# ~of~ budget} \leq K,
% \end{aligned}
% \end{equation}
% where $V^r \subset V_N$ is the candidate nodes to querying using $K$
% budget by $r$ multiple queries of each node and $K^{r}_{p}=[x_1, x_2,
%   \ldots, x_{K/r}]$ is the vector with $0\leq x_i \leq r$ which
% indicates the number of answer ``yes" after $r$ queries for the $i$-th
% $(1\leq i \leq K/r)$ queried node.






% Then, for a given $r$, we first
% need to select the optimal $K/r$ nodes which maximizes $P(v_1 \in
% V^r).$ Next, we need an estimator to maximize the probability in
% \eqref{eqn:OPT}. To do this, we consider MLE by the snapshot $G_N$ and
% queried data $K^{r}_{p}$ due to the lack of priori information about
% the source.  Then, we have the following MLE:
% \begin{equation}\label{eqn:MAP}
% \begin{aligned}
% \hat{v}_{\tt ml}&=\arg\max_{v \in G_N}\mathbb{P}(G_N,
% K^{r}_{p}|v=v_1)\\ &\stackrel{(a)}{=}\arg\max_{v \in
%   G_N}\mathbb{P}(G_N|v=v_1)\mathbb{P}(K^{r}_{p}|v=v_1),\\
% \end{aligned}
% \end{equation}
% where $(a)$ is from the fact that $G_N$ and $K^{r}_{p}$ are independent.

%The first term in \eqref{eqn:MAP} can be obtained by $R(v,G_N)$ from
%\eqref{eqn:ML} easily hence, it remains to find the second term. To
%obtain this, we need to consider the following two cases (a) $v \in
%V_r$ and (b) $v \notin V_r$. First, if $v\notin V_r$ then the
%probability $P(K^{r}_{p}|v=v_1)$ is same for all $v \notin V_r$. Let
%$w$ be the infected node with maximum rumor centrality in $V_{r}^{c}$
%and let $P(v,r):=P(K^{r}_{p}|v=v_1)$ then for a given $r,$ the MLE is
%given by \begin{equation}\label{eqn:MAP2} \begin{aligned}
%\hat{v}_{\tt ml}&=\arg \max_{v\in V_{r} \cup
%\{w\}}R(v,G_N)P(v,r).\\ \end{aligned} \end{equation}

\smallskip
\noindent{\bf \em Challenges.} We now explain the technical challenges
in solving {\bf OPT}. To that end, let us
consider the following sub-optimization in {\bf OPT} for a fixed $ 1\le
r \le K$:
\begin{align}\label{eqn:subOPT}
% \displaystyle
\text{\bf SUB-OPT:} &  \quad \max_{C_r}
  \max_{v \in C_r} \bprob{G_N,A_{r} | v=v_1}.
\end{align}
Then, the following proposition provides the solution of {\bf SUB-OPT}.
\begin{proposition}
  Construct $C_r^*$ by including the $K/r$ nodes in the decreasing order
  of rumor centrality. Then, $C_r^*$ is the solution of {\bf SUB-OPT}.
\end{proposition}

\smallskip
Despite our knowledge of the solution of {\bf SUB-OPT},
solving {\bf OPT} requires an analytical form of the objective value of
{\bf SUB-OPT} for $C_r^*$ to find the optimal repetition count, say
$r^\star.$ However, analytically computing the detection probability for
a given general snapshot is highly challenging due to the following
reasons. We first note that
\begin{align}
  \label{eq:trade}
&\max_{v \in C_r} \bprob{G_N,A_{r} | v=v_1} \cr
& =  \max_{v \in C_r} \bprob{G_N,A_{r}|v=v_1, v_1 \in C_r} \times \prob{v_1 \in
  C_r}.\cr
& =  \underbrace{\prob{v_1 \in  C_r}}_{(a)} \times \underbrace{\max_{v \in C_r} \bprob{G_N,A_{r}| v=v_1, v_1 \in C_r}}_{(b)},
\end{align}
where we will discuss the analytical challenges in $(a)$ and $(b),$
respectively.

First, the term $(a)$ is difficult to analyze, because
\note{....}. Second, to see the challenging in $(b)$, we first observe
that using the independence between $G_N$ and $A_r,$ by letting the
event ${\cal A}(v) = \{v=v_1, v_1 \in C_r\},$
\begin{align}
\label{eq:2}
\hat{v} &= \arg \max_{v \in C_r} \bprob{G_N,A_{r} \mid  {\cal A}(v)} \cr
&= \arg \max_{v \in C_r} \bprob{A_r
  \mid {\cal A}(v)} \times \bprob{G_N\mid {\cal A}(v)}. 
\end{align}
Then, the node $\hat{v}$ maximizing $(b)$ is the node $v$ 
that has the maximum {\em weighted} rumor centrality where the weight is 
$\prob{A_r| {\cal A}(v)}$. As opposed to the case of characterizing the
rumor center in the non-weighted setup, as in \cite{shah2010},
analytically obtaining or graphically characterizing $\hat{v}$ in this
weighted setup is hard, thus which value of $r$ maximizes the detection
probability as formulated in {\bf OPT}. 

% However, obtaining the exact detection probability
% by considering this weight is quite complex because we need to all possible
% sample data after querying. 

%\begin{align}
%  \label{eq:2}
%&  \bprob{v=v_1|G_N,A_{r}, v_1 \in C_r}\cr
%&=  \bprob{v=v_1|G_N, v_1 \in C_r} \times \bprob{v=v_1|A_{r}, v_1 \in
%  C_r},
%\end{align}


% \begin{align}
%   \label{eqn:MAP}
%   \hat{v}_{\tt ml}&=\arg\max_{v \in G_N}\mathbb{P}(G_N,
%                     K^{r}_{p}|v=v_1)\\ &\stackrel{(a)}{=}\arg\max_{v \in
%                                          G_N}\mathbb{P}(G_N|v=v_1)\mathbb{P}(K^{r}_{p}|v=v_1),\\
% \end{align}
% where $(a)$ is from the fact that $G_N$ and $K^{r}_{p}$ are independent.


\begin{comment}
First, it is not easy to find the optimal set $V^r$ for a given budget
$K$ because we do not know what the best strategy to select the set
which maximizes the probability of containing the source. Second, for
calculating the MLE, the first term in \eqref{eqn:MAP} can be obtained
by $R(v,G_N)$ from \eqref{eqn:ML} easily but, the probability
$\mathbb{P}(K^{r}_{p}|v=v_1)$ is quite complex because we have to
consider the all possible cases as varying $r$ which output the data of
each nodes in $V^r$. To handle these issues, we first provide an optimal
solution in \eqref{eqn:OPT} for a given $r$. To see this, consider the
following proposition.
\end{comment}

One can numerically compute it, which, however, needs to generate a lot
of $A_r$ samples (one sample requires a vector of answers for $K$
questions).  Motivated by this, we propose an algorithm producing an
approximate solution of {\bf OPT}. The key of our approximate algorithm
is to choose $C_r$ that allows us to analytical compute the detection
probability for a given $r$ so as to compute $r$ easily, yet its
performance is close to that of {\bf OPT}.

% \begin{equation}\label{eqn:trade}
% \begin{aligned}
% \mathbb{P}(&\hat{v}_{\tt ml}=v_1 |G_N,A_r)\\
% & =\mathbb{P}(\hat{v}_{\tt ml}=v_1|G_N,A_r,v_1 \in C_r)\mathbb{P}(v_1 \in C_r).\\
% \end{aligned}
% \end{equation}

% more simple algorithm
% that three key components should be smartly designed to achieve high
% detection probability: (a) which nodes do we choose as a candidate set
% including the true rumor source, (b) how do we balance between the size
% of candidate set and the query repetition times, and (c) in the nodes
% claiming the rumor source after all the queries, how do we finally
% estimate the source. Our proposed algorithm is designed by considering
% these three facts with simple manner.


\begin{comment}
However, to obtain the optimal solution in \eqref{eqn:OPT}, there are
some challenging issues. First, it is not easy to find the optimal set
$V^r$ for a given budget $K$ because we do not know what the best
strategy to select the set which maximizes the probability of
containing the source. Second, for calculating the MLE, the first term
in \eqref{eqn:MAP} can be obtained by $R(v,G_N)$ from \eqref{eqn:ML}
easily but, the probability $\mathbb{P}(K^{r}_{p}|v=v_1)$ is quite
complex because we have to consider the all possible cases as varying
$r$ which output the data of each nodes in $V^r$. To handle these
issues, we first provide an optimal solution in \eqref{eqn:OPT} for a
given $r$. To see this, consider the following proposition.

\smallskip
\begin{proposition}\label{proposition:optimalN}
For a given $G_N$, suppose $v(i)$ be the infected node with $i$-th
largest rumor centrality in $V_N$ and let $V_K :=\{v(1),\ldots,
v(K)\}$. Then,
\begin{equation}\label{eqn:opt}
\begin{aligned}
\mathbb{P}(v_1 \in V_K)\geq \mathbb{P}(v_1 \in V),
\end{aligned}
\end{equation}
for any subset $V\subset G_N$ with $|V|=K$.
\end{proposition}
\smallskip
This result implies that it is the optimal for choosing the set which
maximizes the probability of containing source when the size of
candidate set is $K$. We will provide the proof of this in
Section~\ref{sec:proof}. Based on this result, for a given $K/r$
queried nodes, we have
\begin{equation}\label{eqn:trade}
\begin{aligned}
\mathbb{P}(&\hat{v}_{\tt ml}=v_1 |G_N,K^{r}_{p})\\
& =\mathbb{P}(\hat{v}_{\tt ml}=v_1|G_N,K^{r}_{p},v_1 \in V^r)\mathbb{P}(v_1 \in V^r).\\
\end{aligned}
\end{equation}
Hence, from the result in Proposition~\ref{proposition:optimalN}, it
is an optimal solution of \eqref{eqn:OPT} for a given $r$ which
selects the candidate set $V^r$ by order of the rumor centrality and
find the source by MLE after queries. However, unfortunately, it is
technically challenging to obtain tractable analytical results for the
candidate set choice based on rumor centrality, because it is not easy
to characterize the probability $\mathbb{P}(v(i) = v_1)$ for obtaining
the probability that $\mathbb{P}(v_1 \in
V^r)=\sum_{i=1}^{K/r}\mathbb{P}(v(i) = v_1)$. Furthermore, to obtain
the solution in \eqref{eqn:OPT}, we have to consider all possible $r$
which maximizes the detection probability because if we increase $r$
to obtain better probability by the MLE in \eqref{eqn:trade}, the
detection probability $\mathbb{P}(v_1 \in V^r)$ becomes decreasing due
to the reducing of the size for candidate set $V^r$.
\end{comment}

\begin{algorithm}[t!]
 \caption{Estimation for Simple Batch Querying}
\label{alg:noninteractive}
 \KwIn{Rumor set $G_N$, budget $K$, degree $d$, and truth probability
   $p>1/2$} \KwOut{Estimator $\hat{v}$}
% \vspace{-0.5cm}\separator
$C_r = \hat{V} = \emptyset$\;
Calculate the rumor centrality $R(v, G_N)$ for all $v \in G_N$ as in
\cite{shah2010} and let $ s \leftarrow \arg\max_{v \in V_N} R(v, G_N)$\; 
Set the repetition count $ r \leftarrow \left \lfloor 1+\frac{(1-p)\log K}{2e\log(d-1)}\right\rfloor$ \; 
% $ s \leftarrow \arg\max_{v \in V_N} R(v, G_N)$\; 
Construct a candidate
set $C_r$ by including each node $v$ that satisfies $d(v,s)\leq l
,$ where $l=\frac{\log\left(\frac{K(d-2)}{rd}+2\right)}{\log(d-1)}$ and 
$d(v,s)$ is the hop distance between nodes $v$ and $s$\;
 % Compute the maximum distance $l$ from \eqref{eqn:l} and assign a
 % set $V_l$ which consists of satisfying $d(v,s)\leq l$ for all nodes
 % $v \in V_N$\;
 % l=\frac{\log\left(\frac{K(d-2)}{rd}+2\right)}{\log(d-1)}.

% $\hat{V} \leftarrow \emptyset$ \;
\For{each $v \in C_r$}{
% $\mu(v)\leftarrow 0$\;
Count the number of ``yes'' (i.e., I am the rumour source) for the
identity question, stored at $\mu(v),$ and if $\mu(v)/r \geq 1/2$ then
include $v$ in $\hat{V}$\; }
% \While{$r\geq 1$}{ $v$ selects a random variable $X\sim U(0,1)$\;
%    \If{$X\leq v(p)$}{ $\mu(v)\leftarrow \mu (v) +1$\;} }

%   \If{$\mu(v)/r \geq 1/2$}{ $\hat{V} \leftarrow \hat{V} \cup
%    \{v\}$\;} }
\While{$K-r|C_r|\geq r$}{ Select a node $v$ satisfying $d(v,s)= l+1$
  uniformly at random\; Do the same procedure in Lines 6-7\; }

 \If{$\hat{V}=\emptyset$}{ $ \hat{v} \leftarrow \arg\max_{v\in C_r}
   R(v, G_N)$\; } \Else{ $ \hat{v} \leftarrow \arg\max_{v\in\hat{V}}
   R(v, G_N)$\; }
% Return $\hat{v}=s$\;
\end{algorithm}

\subsection{Algorithm based on Hop Distance and Majority Rule}

We now propose an algorithm that overcomes the afore-mentioned
challenges in $(a)$ and $(b)$ in \eqref{eq:trade}.  The key idea is that
for $(a)$ we adopt a {\em hop-distance based selection} of the candidate
set $C_r$ and for $(b)$ we simply apply a {\em majority-based rule}, as
will be clarified soon. 

We first formally describe our algorithm in {\bf
  Algorithm~\ref{alg:noninteractive}} and explain how it operates,
followed by presenting the rationale behind it: we first calculate the
rumor centrality of all nodes in $G_N$ (Line 1), where $s$ is set to be
the rumor center. Then, we appropriately choose the repetition count as
in Line 3, and construct the candidate set $C_r$ by the nodes within the
hop-distance given in Line 5 from the rumor center $s.$ Next, for each
node in $C_r,$ we ask the identity question $r$ times, and count the
number of ``yes''es in $\mu(v)$ (Lines 5-6). Using this, we filter out
the candidate set $C_r$ and construct $\hat{V}$ by including the nodes
with $\mu(v)/r \geq 1/2$ (majority rule), i.e., the nodes with higher
chance to be the rumor source.  When $K$ is not a multiple of $r,$ we
handle the remaining $K-r |C_r|$ nodes as in Lines 7-9. Finally we
choose the node in $\hat{V}$ with highest rumor centrality, where if
$\hat{V} = \emptyset,$ we simply do the same task for $C_r.$


% based on the hop-distance from the rumor center as
% follows (Line 5): we contain  containing all infected nodes within
% the distance to the rumor center



% chooses $s$ as the rumor center. Next, it
% selects the repetition count $r$ as in line 3 and by using this, it
% constructs a candidate set $V_c$ containing all infected nodes within
% the distance to the rumor center as in line 5.  As the second part, in
% line 6-7, it queries to all node $v \in V_c$ by $r$ times then it put
% the node to $\hat{V}$ if te number of "yes" is more than half of $r$.
% Then, if there are remained budget which is greater than $r$, then the
% algorithm selects a node at the one hop


% We appropriately consider (a), (b), and (c) and proposed the detection
% algorithm, described in {\bf Algorithm~\ref{alg:noninteractive}},
% followed by its rationale.

%In terms of choosing the candidate set, one can propose the method of
%prioritizing the nodes with higher rumor centrality quantified by
%$R(v,G_N).$ In fact, we can prove
%Proposition~\ref{proposition:optimalN} which states that for any
%fixed $r$ and for any $p,$ choosing $K/r$ candidate nodes with
%decreasing order of their rumor centralities outperforms any other
%mechanism in terms of detection probability, whose proof is presented
%in
%Section~\ref{sec:proof}.  \begin{proposition}\label{proposition:optimalN}
%Suppose $v(i)$ be the infected node with $i$-th largest rumor
%centrality in $V_N$ and let $V_K :=\{v(1),\ldots,
%v(K)\}$. Then, \begin{equation}\label{eqn:opt} \begin{aligned}
%\text{Pr}(v_1 \in V_K)\geq \text{Pr}(v_1 \in
%V), \end{aligned} \end{equation} for any subset $V\subset G_N$ with
%$|V|=K$.  \end{proposition} \smallskip

% This consists of three parts. In the first part (line 1 - 4), from
% the given snapshot $G_N$, it calculates the rumor centrality
% $R(v,G_N)$ by using the technique in \cite{shah2010} and selects the
% maximum centrality node $s$.

% We first start with simple batch querying scenario. This
% querying scheme involves simultaneous guessing multiple nodes as rumor
% source. If any one node matches with rumor source, the estimation is
% successful. However, there may be many schemes to select such multiple
% nodes with different detection performance. One of such scheme, we may
% consider the rumor centrality based one which achieves the optimal
% performance as follows.

% This result indicates that the selection scheme based on the rumor
% centrality is the optimal for the non-interactive querying. We will
% provide the proof in Appendix. However, due to the
% tractability issue for obtaining $\text{Pr}(v_1 \in V_K)$, instead
% of using this scheme, we use more simple and quite good scheme as
% following definition.

% \smallskip \begin{definition} When the infected set $V_N\subset V$
% is given, we say that a particular node $v \in V_N$ satisfies
% \emph{$L$-hop criterion} if following inequality
% holds \begin{equation*} d(v_{RC}, v)\leq L, \end{equation*} where
% $d(v_{RC}, v)$ is the hop-distance from the rumor center $v_{RC}$
% for $L\geq 0$.  Moreover, we let $V_{L} \subseteq V_N$ be the set of
% nodes which satisfies $L$-hop
% criterion.  \label{def:L-criterion} \end{definition} \smallskip


\smallskip
\noindent{\bf \em Rationale.} We now provide the rationale of {\bf
  Algorithm 1} from the perspective of how we handle the
analytical challenges in \eqref{eq:trade}  so as to approximately solve
{\bf OPT} in an approximate manner. 

\smallskip
\begin{itemize}
\item[$\circ$] {\em Hop Distance based $C_r$ selection:} Selecting 
  $C_r$ based on the distance from the rumor center, rather than based
  on the sorted rumor centrality permits us to have the closed form of
  $\prob{v_1 \in C_r}.$ This is because \note{.......}.\vspace{2cm}


\item[$\circ$] {\em Construction of filtered candidate set $\hat{V}$
    from querying:} Instead of using the exact weight rumor centrality,
  We use more simple scheme to approximate this. Consider that if the
  node $v_i$ output the querying data by $x_i$ then for $r$ times
  questions, from the fact that $p>1/2$, we know that if $x_i \geq r/2$
  then the weight becomes high and vise versa. Since we will find the
  maximum weighted centrality nodes in $C_r$, we set
  $\bprob{A_r|{\cal A}(v)}=1$ if $x_i \geq r/2$ and $\bprob{A_r|v_i}=0$
  if $x_i < r/2$.
\end{itemize}

Using the above approximation techniques, we are able to have the closed
and approximate form of {\bf SUB-OPT}, which allows us to compute the
best $r^\star$ that maximizes the detection probability as in
$r^*= \left \lfloor 1+\frac{(1-p)\log K}{2e\log(d-1)}\right\rfloor.$

% Due to this reason, we analytically study and
% derive the ``optimal'' value of $r^*= \left \lfloor 1+\frac{(1-p)\log
%   K}{2e\log(d-1)}\right\rfloor$ that maximizes the detection
% probability under our framework, which is thus used in our
% algorithm. By selecting this proper $r$, we avoid the issue that needs
% to consider all possible $r$ to maximizes this probability in
% \eqref{eqn:OPT}.

% \note{rationale} \note{how do we simply the complex parts...}

% \smallskip
% \noindent{\bf \em (a) Hop-distance based $C_r$ selection:}
% \note{we solve (a), hop-distance, thus, we can compute... hop-based why
%   easy to compute......high-level..., as will be presented in Theorem 1.},




---------------------------------------
In
our algorithm, we first choose the node with the largest rumor
centrality $s$ (Line 3), and select the query repetition count $r$ as
in Line 3.  For a given budget $K,$ the size of the candidate set can
be $K/r,$ where we choose the queriee candidate set based on their hop
distance to $s,$ where the distance is appropriately chosen such that
we use the budget $K/r$ (Line 5).  We believe that this scheme is a
good approximation because the source is nearby the rumor center with
high probability, which is also quantified for the case of truthful
users by \cite{Khim14} as following lemma.
By choosing this set as a candidate set, we address the
first issue (a) that how to choose the candidate set properly because
this is very simple scheme and has a good detection performance as in
\cite{Khim14} which is derived by rumor centrality.
\begin{comment}
 which is derived by MLE calculations of rumor centrality. Hence, we
 use this criteria for selecting the candidate set. Clearly, the
 detection probability will increase compared to the single point
 estimation for the case of $p_v=1$ for all $v\in V_N$.  However, if
 $p_v<1,$ we do not know how much query can guarantees the detection
 performance which is depends on the number of queries $K$ and the
 probability $p_v$. For the tractability of analysis, we consider the
 case of $p_v=p$ for all node $v\in V_L$. In the following sections,
 we will introduce the proposed simple batch querying algorithm and
 derive the performance guarantee that how many budget is required to
 guarantee the target probability under $d$-regular trees.
\end{comment}

%\smallskip
%\begin{lemma}(\cite{Khim14})\label{lem:L-hop}
%For a $d$-regular tree ($d\geq 3$), let $V_L$ be the set of infected nodes in
%$L$-hop distance to the rumor center. Then, for $L\geq 2$,
%\begin{equation}\label{eqn:L-hop}
%    \begin{aligned}
%   \mathbb{P}(v_1 \notin V_L)\leq c e^{- \frac{L}{2}\log L}.
%    \end{aligned}
%  \end{equation}
%where $c = 7(d+1)/d.$
%\end{lemma}
%\smallskip
%This result\footnote{This result has been simplified by constant term from
%the result in \cite{Khim14}.} implies that the probability of distance between the
%source and rumor center decaying exponentially with respect to the
%distance.
%For a given budget $K$, there may be many schemes to use these budget
%in the non-interactive querying to ontain a proper detection
%performance. For example, some scheme uses all the budget only to
%assign the maximal candidate set by single query to each nodes in the
%set. However, there may be a scheme that uses a portion of budget to
%assign the candidate set and uses the remained budget to ask multiple
%queries for increasing the quality of answer for each node.

% \smallskip
% \noindent{\bf \em (b) Choice of $r$.}

Next, to consider second issue (b), the right value of the query
repetition count $r$ is of critical importance in achieving high
detection probability, where $r$ trade offs the size and the quality
of the selected queriees. For example, when $r=1,$ i.e., we choose a
large candidate set, but only one query can be asked for each node in
the candidate set, in which case, we have to estimate the rumor source
from too many possible candidate nodes without chance of confirming
who is close to the true rumor source.  Hence, the detection
probability can not close to one even for sufficiently large budget
$K$. Due to this reason, we analytically study and
derive the ``optimal'' value of $r^*= \left \lfloor 1+\frac{(1-p)\log
  K}{2e\log(d-1)}\right\rfloor$ that maximizes the detection
probability under our framework, which is thus used in our
algorithm. By selecting this proper $r$, we avoid the issue that needs
to consider all possible $r$ to maximizes this probability in
\eqref{eqn:OPT}. Then, by using this $r$, we calculate the maximal
distance $l<L$ from the rumor center. Indeed, from the fact that there
are $K_l:=\frac{d(d-1)^{l}-2}{d-2}$ nodes in the distance $l<L$ from
the rumor center of the $d$-regular tree, for a given $K$ and $r$, we
have $K\geq r K_l$. By using this, we obtain
$l=\lfloor\log\left(\frac{K(d-2)}{rd}+2\right)/ \log(d-1)\rfloor$.
%We show that this probability is strictly less than one for $r=1$
%for arbitrary $K$ by MLE as following lemma.
%
%\smallskip
%\begin{lemma}\label{lem:r1}
%  Consider the $d$-regular tree and MLE algorithm in \eqref{eqn:MAP}
%  for the single querying ($r=1$) with probability $p$. Then for any
%  $K\geq 1$, the detection probability of MLE is upper bounded by
%\begin{equation}\label{eqn:upper}
%   \begin{aligned}
%  \mathbb{P}(\hat{v}_{\tt ml}=v_{1})\leq \alpha_d+(1-\alpha_d)(p^2
%  +(1-p)^2),
%   \end{aligned}
% \end{equation}
% where $\alpha_d :=\lim_{N\rightarrow \infty} \mathbb{P}(v_{RC}=v_1)$
% be the probability that the rumor center is the source when the
% number of infected nodes goes to infinity which is given by
% \cite{shah2012}
%\begin{align*}
%\alpha_{d}=\begin{cases} \qquad\qquad
%0&\mbox{if}~d=2\\ 1-d\left(1-\emph{I}_{1/2}\left(\frac{1}{d-2},\frac{d-1}{d-2}\right)\right)
%&\mbox{if}~d\geq 3.
%\end{cases}
%\end{align*}
%Here, $I_\alpha (a, b)$ is a regularized incomplete Beta function: % which
%                                                                   % is
%\begin{equation*}
%I_\alpha (a, b) = \frac{\Gamma(a+b)}{\Gamma(a)\Gamma(b)} \int_0^\alpha
%t^{a-1} (1-t)^{b-1}dt,
%\end{equation*}
%where $\Gamma(\cdot)$ is the standard Gamma function. Furthermore,
%$\alpha_{d}$ has the value between zero to 0.307 for any $d\geq 2$.
%\end{lemma}
%\smallskip
%From this result, we see that if $p=3/4$ then $\mathbb{P}(\hat{v}_{\tt
%  ml}=v_{1})$ can not beyond 0.75. We will provide the proof of this
%lemma in the Appendix.


\begin{comment}
In fact, Theorem~\ref{thm:r1} states a poor detection probability for
a wrong choice of $r$, implying that it is impossible to obtain high
detection quality whatever the budget size $K$ is.

\begin{theorem}\label{thm:r1}
  Consider the $d$-regular tree and MLE algorithm with the single
  noisy feedback with probability $p$. Then for any $K\geq 1$, the
  detection probability of MLE is upper bounded by
\begin{equation}\label{eqn:upper}
   \begin{aligned}
  \text{Pr}(\hat{v}_{\tt ml}=v_{1})\leq \alpha_d+(1-\alpha_d)(p^2
  +(1-p)^2).
   \end{aligned}
 \end{equation}
\end{theorem}

First, this result implies that if there is a noisy feedback for the
non-interactive querying, then the number of budget can not make the
probability close to one even though for the extremely large $K$
because when $p\neq 1$ in \eqref{eqn:upper} then this is strictly
small than one. For example, if $p=3/4$ then $\text{Pr}(\hat{v}_{\tt
  ml}=v_{1})$ can not beyond 0.75.
\end{comment}

% A few interpretations of Theorem~\ref{thm:noninteractive0} are in
% order.  % as in

% \smallskip \begin{compactenum}[(a)] \item First, this result implies
% that if there is a noisy feedback for the non-interactive querying,
% then the number of budget can not make the probability close to one
% even though for the extremely large $K$ because when $p\neq 1$ in
% \eqref{eqn:upper} then this is strictly small than one. For example,
% if $p=3/4$ then $\text{Pr}(\hat{v}_{\tt ml}=v_{1})$ can not beyond
% 0.75.  \item Second, we see that this upper bound has the minimum at
% $p=1/2$ \ie there is no further information by the querying. In
% addition to this, the upper bound of probability is symmetric with
% respect to $p$ because the information is same except $p\neq
% 1/2$.  \item Third, the right term in \eqref{eqn:upper} is the gain
% of the non-interactive querying since $\alpha_d$ is the probability
% of MLE when there is no querying.

% \end{compactenum} \smallskip This result implies that if there is a
% noisy feedback for the non-interactive querying, then the number of
% budget can not make the probability close to one even though for the
% extremely large $K$ because when $p\neq 1$ in \eqref{eqn:upper} then
% this is strictly small than one.  To overcome this issue, we
% introduce a scheme which is a kind of multiple query to each node in
% the candidate set.

\smallskip
\noindent{\bf \em (b) Filtering and final estimation.}

\note{how (5) is approximated by majority based filtering and RC-based selection...}
Instead of using the exact weight rumor centrality, We use more simple scheme 
to approximate this. Consider that if the node $v_i$ output the querying 
data by $x_i$ then for $r$ times questions, from the fact that $p>1/2$, we know that if $x_i \geq r/2$ 
then the weight becomes high and vise versa. Since we will find the
maximum weighted centrality nodes in $C_r$, we set $\bprob{A_r|v_i}=1$ if $x_i \geq r/2$
and $\bprob{A_r|v_i}=0$ if $x_i < r/2$. This is the explanation of 
line 6-14 in the Algorithm~ \ref{alg:noninteractive}.
From
the fact that each queried node answer the truth with probability $p$
for each time, the algorithm cumulates the number of reveals as the
rumor source. In the line 7, $\mu(v)$ is the total count of revealing
itself as the rumor source for the infected node $v \in V_c$. If
$\mu(v)$ is greater than half of $r$ then it selects the node as the
candidate node and put the node in the candidate set $\hat{V}$. From
the fact that $p>1/2$, the source will be in $\hat{V}$ with
probability larger than $p$ and other queried node will not be in this
set with probability larger than $p$. Hence, it is rational to search
the source in the set $\hat{V}$.  In addition to this, since the
candidate set is defined by the distance from the rumor center, there
may be remained budget after selecting $r$ and $l$ for a given budget
$K$. Hence, we use this budget for asking additional $l+1$ hop nodes
uniformly at random in line 8-10.  Finally, in the third part (line
11-14), the algorithm chooses the node with maximum centrality in the
selected candidate set $\hat{V}$. If this set is empty, then it
chooses the node with maximum centrality in the original set $V_c$.

\begin{comment}
In this algorithm, even though we use the $L$-hop criteria to select
the candidate set for simplicity, as described before, this is
somewhat nice compared to the optimal selection which is based on the
rumor centrality.  In addition to this, we derive the optimal $r$
instead of using just one query ($r=1$) so that the performance of
detection increases. In Appendix, we derive that if there is only one
query to each node, then the detection probability can not beyond the
probability $p$ even for sufficiently large budget $K$ in this
algorithm \footnote{We also prove that the detection probability by
  using MLE can not goes to one for any $K$.}. Finally, we use also
the information of snapshot which is the rumor centrality so that it
guarantees the proper estimation among the nodes in the candidates
set.
\end{comment}

%From the result in the previous section, we know that the single
%feedback has a limitation for detecting the source with arbitrary
%close to one for any budget $K$ because the queries can not increase
%the probability $p$ for each nodes. Hence, we tackle this by using
%multiple independent feedbacks from the queried node which can
%increases the probability $p$ by simple majority based decision rule.



\subsection{Detection Performance}

As a main result, we state the following theorem for the analytic
performance of Algorithm~\ref{alg:noninteractive}. We first obtain the
lower bound of detection probability for a given $r$, then by using
this, we find the optimal $r^*$ and derive that for a given
$\delta>0$, how many query budget is required to achieve the detection
probability at least $1-\delta$ as follows.

\smallskip
\begin{theorem}
For $d$-regular trees ($d\geq 3$), the detection probability of the Simple Batch
Querying ($p>1/2$) for given $K, p$ and $r$ is given by
\begin{equation}\label{eqn:detect}
    \begin{aligned}
\mathbb{P}(\hat{v}=v_1)\geq\frac{r+p}{r+1}\left(1-c\cdot exp\left(-h_d
(K,r)/2\right)\right),\\
    \end{aligned}
  \end{equation}
where $h_d
(K,r):=\frac{\log\left(\frac{K}{r}\right)}{\log(d-1)}\log\left(
\frac{\log\left(\frac{K}{r}\right)}{\log(d-1)}\right)$ and $c = 7(d+1)/d.$
Furthermore, by obtaining the optimal $ r^*$ in \eqref{eqn:detect}, we have for
sufficiently small $\delta>0,$ if
\begin{equation}\label{eqn:elower}
    \begin{aligned}
     K\geq \frac{c(2/\delta)}{p^2\log (\log (2/\delta))},
    \end{aligned}
  \end{equation}
then the detection probability is at least $1-\delta$ where
$c=4(d-1)/(d-2)$ is a constant depends on $d$.
\label{thm:noninteractive}
\end{theorem}
\smallskip
This results indicates that if there is untruthful answer with
probability $p>1/2$, then we need $1/p^2$ times more budget of
querying to satisfy the same target probability compared to the case
of $p=1$ which is also derived in \cite{Khim14}. If $p\simeq 1/2$ then
it needs about 4 times more budget to guarantee the same target
detection probability. Furthermore, if $p=0.6$ then it needs $K\geq 684$
budget to achieve at least 95\% accuracy for detection probability
when $d=3$.






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proof_jy.tex <==
% \section{Estimating Rumor Sources with Querying}

\section{Proofs of Results}
\label{sec:proof}
In this section, we will provide the proof of Propositions and Theorems.

\subsection{Proof of Proposition~\ref{prop:simple_prob}}

To obtain the lower bound of the detection probability, consider that for a given
$r$, we have
the detection probability as
\begin{equation}\label{eqn:detection}
    \begin{aligned}
      \mathbb{P}(\hat{v}=v_{1})&=\mathbb{P}
      (\hat{v}=v_1,v_1 \in V_{l}) \\ &=\mathbb{P}
      (\hat{v}=v_1|v_1 \in V_{l})\cdot\mathbb{P}(v_1 \in
      V_{l}) \\
    \end{aligned}
  \end{equation}
where $V_l$ be the set of infected nodes which distance to the rumor 
center is $l\leq L$. To obtain the probability $\mathbb{P}(v_1 \in V_{l})$, 
we consider the following lemma.

\smallskip
\begin{lemma}(\cite{Khim14})\label{lem:L-hop}
For a $d$-regular tree ($d\geq 3$), let $V_L$ be the set of infected nodes in
$L$-hop distance to the rumor center. Then, for $L\geq 2$,
\begin{equation}\label{eqn:L-hop}
    \begin{aligned}
   \mathbb{P}(v_1 \notin V_L)\leq c e^{- \frac{L}{2}\log L}.
    \end{aligned}
  \end{equation}
where $c = 7(d+1)/d.$
\end{lemma}
\smallskip
This result\footnote{This result has been simplified by constant term from
the result in \cite{Khim14}.} implies that the probability of distance between the
source and rumor center decaying exponentially with respect to the
distance. Hence, it remains to find the probability $\mathbb{P}
(\hat{v}=v_1|v_1 \in V_{l})$ in \eqref{eqn:detection}. To do this, 
consider that 
\begin{equation}\label{eqn:detection1}
    \begin{aligned}
    \mathbb{P}(\hat{v}=v_1&|v_1 \in V_{l})=\mathbb{P}(v_1 \in \hat{V}, v_1 =v_{LRC}|v_1 \in V_{l})\\
    &=\mathbb{P}(v_1 \in \hat{V}|v_1 \in V_{l})\mathbb{P}(v_1 =v_{LRC}|v_1 \in V_{l}),\\\\
    \end{aligned}
  \end{equation}
where $v_{LRC}$ is the \emph{Local Rumor Center} (LRC) which is the nodes with maximum rumor centrality in 
$\hat{V}$. To obtain the first term in \eqref{eqn:detection1}, let
 $\hat{p}:=\mathbb{P}(v_{1} \in \hat{V}|v_1 \in V_{l})$ which is the probability that the source
is in the final candidate set by the majority-based decision rule in
the Algorithm ~\ref{alg:noninteractive} and let $X_i(v)$ be the random
variable with which takes $+1$ if the queried node answer ``yes" and
takes $0$, otherwise for a given $r\geq 1$. Then, one can easily check that this follows the
Bernoulli random variable with probability $p>1/2$.  Let
$Z(v)=\sum_{i=1}^{r}X_i (v)$ then, we have
\begin{equation}\label{eqn:majority}
    \begin{aligned}
     \hat{p}:=\mathbb{P}\left(Z(v)\geq r/2\right)&=\sum_{j=0}^{\lfloor
       r/2\rfloor}\binom{r}{j}(1-p)^{j}p^{r-j}\\ &=I_{p}(r-\lfloor
     r/2\rfloor, \lfloor r/2\rfloor+1),
    \end{aligned}
  \end{equation}
where $I_{p}(\cdot)$ is the regularized incomplete beta
function. Clearly, this probability becomes larger than $p$ when
$p>1/2$ and it goes to one for $r$ increases. Next, 
we need to obtain the second term in \eqref{eqn:detection1}. To do this,
consider the following lemma. 

\smallskip
\begin{lemma}(\cite{dong2013})\label{lem:suspect}
For a $d$-regular tree ($d\geq 3$), suppose that there are $k$ suspect nodes which
contains the rumor source and let $\varphi_{d}(k):=\lim_{N\rightarrow
  \infty} \mathbb{P}(\hat{v}_{MAP}=v_1)$.  Then
\begin{equation}\label{eqn:suspect}
    \begin{aligned}
      \varphi_{d}(k) \geq 1-\frac{2(k-1)}{k}\left(1-I_{1/2} \left(
      \frac{1}{d-2}, \frac{d-1}{d-2} \right)\right).
    \end{aligned}
  \end{equation}
Here, $I_\alpha (a, b)$ is a regularized incomplete Beta function:
\begin{equation*}
I_\alpha (a, b) = \frac{\Gamma(a+b)}{\Gamma(a)\Gamma(b)} \int_0^\alpha t^{a-1} (1-t)^{b-1}dt,
\end{equation*}
where $\Gamma(\cdot)$ is the standard Gamma function.
\end{lemma}
\smallskip
The inequality in \eqref{eqn:suspect} becomes the equality if the
suspect set is connected. This result provides the detection
probability of MAPE when the size of suspect set is given. 
In other
words, if there are $k$ infected nodes in the suspect set then the
probability that the local rumor center is the source
is given by \eqref{eqn:suspect}. Let $V_{l,\hat{p}}$ be
the set of final candidate node in $V_l$ after $r$ queries under the
probability $p>1/2$ and let $\varphi_{d}(V_{l,\hat{p}})$ be the
detection probability when the estimator chooses the maximum rumor
centrality node among $V_{l,\hat{p}}$ then, we have $\mathbb{P}
(\hat{v}=v_1|v_1 \in
V_{l})=\hat{p}\cdot\varphi_{d}(V_{l,\hat{p}}).$ From
\eqref{eqn:detection}, the detection probability is given by
\begin{equation}\label{eqn:result1}
    \begin{aligned}
     \mathbb{P}(&\hat{v}=v_{1})\geq\hat{p}\cdot\varphi_{d}(V_{l,\hat{p}})\left(1-c
     \cdot e^{-\frac{l}{2}\log l}\right),\\
    \end{aligned}
  \end{equation}
where $c=7(d+1)/d$. However, the first two terms $\hat{p}$ and
$\varphi_{d}(V_{l,\hat{p}})$ are somewhat difficult to handle because
these term contains the incomplete beta functions. To simplify the
result, we first consider the following lemma.

\smallskip
\begin{lemma}
For a given $r$, if $p>1/2$ then
\begin{equation*}
\begin{aligned}
\hat{p}\geq p+(1-p)(1-e^{-p^{2}\log r}),
\end{aligned}
\end{equation*}
where $\hat{p}$ is given by \eqref{eqn:majority}.
\label{lem:majority}
\end{lemma}
\smallskip
This is more simple form compared to \eqref{eqn:majority} and this
result also shows that how the parameters $p$ and $r$ effect the
changing of the probability $\hat{p}.$ We will provide the proof of
this in the technical paper in []. By multiple queries to each node, the size
of $V_{l,\hat{p}}$ will decrease so that the detection probability
will be larger. Based on this, we also obtain the simple bound for the
probability $\varphi_{d}(V_{l,\hat{p}})$ as follows.

\smallskip
\begin{lemma}
For a $d$-regular tree ($d\geq3$), if $p>1/2$ then
\begin{equation*}
\begin{aligned}
\varphi_{d}(V_{l,\hat{p}})\geq 1-e^{-p^{2}r\log r}.
\end{aligned}
\end{equation*}
\label{lem:noninteractive}
\end{lemma}
In this lemma, the result shows that how fast this probability
converges to one as the function of $r$ and $p$. The proof of this
lemma also will be given in [].  Then, from the results
in Lemma~\ref{lem:majority} and Lemma~\ref{lem:noninteractive}, we
have
\begin{equation*}
\begin{aligned}
\hat{p}\varphi_{d}(V_{l,\hat{p}})&\geq \left(p+(1-p)(1-e^{-p^{2}\log
  r})\right)\left(1-e^{-p^{2}r\log r}\right)\\ &\geq 1- e^{-p^{2}\log
  r}\stackrel{(a)}{\geq} 1-\frac{1-p}{r+1}=\frac{r+p}{r+1},
\end{aligned}
\end{equation*}
where $(a)$ is from the fact that $e^{-p^2\log r}\leq (1-p)/(r+1)$. Next, consider
that
\begin{equation*}
\begin{aligned}
l\log l
&=\frac{\log\left(\frac{K(d-2)}{rd}+2\right)}{\log(d-1)}\log\left(\frac{\log\left(\frac{K(d-2)}{rd}+2\right)}{\log(d-1)}\right)\\ &
\geq
\frac{\log\left(\frac{K}{r}\right)}{\log(d-1)}\log\left(\frac{\log\left(\frac{K}{r}\right)}{\log(d-1)}\right):=h_d
(K,r).\\
\end{aligned}
\end{equation*}
Then, we obtain the following simple form as a lower bound:
\begin{equation}\label{eqn:part1}
\begin{aligned}
\mathbb{P}(&\hat{v}=v_{1})\geq\frac{r+p}{r+1}\left(1-c \cdot exp\left(-h_d
(K,r)/2\right)\right),\\
\end{aligned}
\end{equation}
where $c=7(d+1)/d$ and which proves the first part of Proposition
~\ref{prop:simple_prob}.


\subsection{Proof of Theorem~\ref{thm:noninteractive}}


\smallskip
 Next, we will obtain the optimal $r^*$
which maximizes the detection probability in \eqref{eqn:part1} as
follows.

\smallskip
\begin{lemma}
For $d$-regular tree, if $p>1/2$ then the optimal $r^*$ is given by
\begin{equation*}
\begin{aligned}
r^* \simeq\left\lfloor 1+\frac{(1-p)\log
     K}{2e\log(d-1)}\right\rfloor.
\end{aligned}
\end{equation*}
\label{lem:redundancy}
for a given budget $K$.
\end{lemma}
\smallskip
We will provide the proof of
Lemma~\ref{lem:redundancy} in Section~\ref{sec:proof}. By using these
lemmas, we will provide the required budget to obtain the detection
probability at least $1-\delta$ for a given $\delta >0$. To do this,
we consider the error probability for given $K$ and $p$. The detection
error can be occurred as following two cases. First, the source is not
in $V_l$ and second, the source is in $V_l$ but the estimator can not
find the source. To obtain the probability, let $E_1:=\{d(v_{RC},v_1)
\geq l\}$ be the event for the first case and let $E_2:=\{\hat{v}\neq
v_{1}|d(v_{RC},v_1) < l\}$ be the second case then the error
probability is givne by
\begin{equation}\label{eqn:disjoint}
\begin{aligned}
&\mathbb{P}(\hat{v}\neq v_{1})=\mathbb{P}(E_1 \cup
  E_2)\stackrel{(a)}{=}\mathbb{P}(E_1)+\mathbb{P}(E_2),\\
\end{aligned}
\end{equation}
where $(a)$ is due to the disjoint events of $E_1$ and $E_2$.  The
first error is bounded by $\mathbb{P}(E_1)\leq c\cdot e^{- l\log
  l}$ by Lemma~\ref{lem:L-hop}. To obtain the second error, we use
Lemma~\ref{lem:majority} and Lemma~\ref{lem:noninteractive} such as
\begin{equation*}
\begin{aligned}
\hat{p}\varphi_{d}(V_{l,\hat{p}})&\geq p+(1-p)(1-e^{-p^{2}\log
  r})(1-e^{-p^{2}r\log r})\\ &\geq 1-(1-p)e^{-p^{2}r\log r}.\\
\end{aligned}
\end{equation*}
Hence, by using this, the error probability $\text{Pr}(E_2)$ is
bounded by
\begin{equation*}
\begin{aligned}
\mathbb{P}(E_2) &\leq (1-\hat{p}\cdot\varphi_{d}(V_{l,\hat{p}}))(1-c
\cdot e^{- \frac{l}{2}\log l})\\ &\leq (1-p)e^{-p^{2}r\log r}.
\end{aligned}
\end{equation*}
Then, by combining the probabilities $\text{Pr}(E_1)$ and
$\text{Pr}(E_2)$, we have the total error probability as
\begin{equation*}
\begin{aligned}
\mathbb{P}(\hat{v}\neq v_{1})&=\mathbb{P}(E_1)+\mathbb{P}(E_2)\\ &\leq
(1-p)e^{-p^{2}r\log r}+c\cdot e^{- \frac{l}{2}\log l}.\\
\end{aligned}
\end{equation*}
By using this, let $(1-p)e^{-r\log r} \leq \delta_1 /2$ and $c \cdot
e^{- \frac{l}{2}\log l} \leq \delta_2 /2$ then we can find the minimum number
of budget $K_1$ for the first case and $K_2$ for the second case.  By
the result of Lemma~ \ref{lem:L-hop} in \cite{Khim14}, we obtain that if
$K_2 \geq \frac{c_2 (2/\delta_2)}{\log (\log (2/\delta_2))}$ where 
$c_2 = (d-1)/(d-2)$ then $c
\cdot e^{- \frac{l}{2}\log l} \leq \delta_2 /2$. Hence, as a next step, we
need to show that if $K_1 \geq \frac{c_1 (1-p^2)(2/\delta_1)}{p^2\log
  (\log (2/\delta_1))}$ then $(1-p)e^{-p^{2}r\log r} \leq \delta_1
/2$. To see this, consider the equivalent form as $\frac{e^{p^2 r\log
    r}}{1-p}\geq \frac{2}{\delta_1}$ and taking logarithm to both
sides, then after some manipulations, we have
\begin{equation*}
    \begin{aligned}
    r\log r \geq \frac{(1-p)^2 (1+p)}{p^2}\log
    \left(\frac{2}{\delta_1}\right).
    \end{aligned}
  \end{equation*}
By using the result in Lemma~\ref{lem:redundancy} which is $r=\Theta
((1-p)\log K)$ and by similar approach in \cite{Khim14}, one can check
that if $K_1 \geq \frac{c_1 (1-p^2)(2/\delta_1)}{p^2\log (\log
  (2/\delta_1))}$ where $c_1 = 4(d-1)/(d-2)$ then $(1-p)e^{-p^{2}r\log r} \leq \delta_1 /2$. By
combing these, we have if
\begin{equation*}
    \begin{aligned}
    K&\geq K_1 +K_2 \\ &\geq\frac{c_1 (1-p^2)(2/\delta_1)}{p^2\log
      (\log (2/\delta_1))}+\frac{c_2 (8/\delta_2)}{\log (\log
      (2/\delta_2))}\\ &=\frac{c_1 (1-p^2)(2/\delta_1)}{p^2\log (\log
      (2/\delta_1))}+\frac{c_2 p^2 (2/\delta_2)}{p^2\log (\log
      (2/\delta_2))}\\ &\geq\frac{c(2/\delta)}{p^2\log (\log
      (2/\delta))},\\
    \end{aligned}
  \end{equation*}
then $\text{Pr}(\hat{v}= v_{1})\geq 1-\delta$ where $\delta:=\min \{\delta_1, \delta_2\}$ 
and $c:=\max\{c_1 ,c_2\}=4(d-1)/(d-2)$, respectively. Hence, we complete the
Theorem~\ref{thm:noninteractive}.



\subsection{Proof of Proposition~\ref{prop:inter_prob}}

To prove this, we first obtain the upper bound of the error
probability when $r=1$ \ie only one direction question is allowed. 
After obtaining the result, we easily extend the probability for 
general $r$ which will be provide in later.
From the fact that the interactive querying consists of two kinds of
questions, we assume that $K$ is even \footnote{One can obtain for odd
  $K$ by similar approach. } for the simple analysis. Then, as similar
to the approach in the proof of Theorem~\ref{thm:noninteractive}, we
define two error events $E_1:=\{d(v_{RC},v_1) > K/2\}$ and
$E_2:=\{\hat{v}\neq v_{1}|d(v_{RC},v_1) \leq K/2\}$. Due to the
disjoint of these events, the error probability is represented by
$\mathbb{P}(\hat{v}\neq v_{1})=\mathbb{P}(E_1)+\mathbb{P}(E_2)$.
However, by the result in Lemma~\ref{lem:L-hop}, we have
$\mathbb{P}(E_1)=\mathbb{P}(d(v_{RC},v_1) > K/2)\leq c \cdot e^{-
  K/\log (K/2)},$ where $c=7(d+1)/d$. To obtain the error probability $\mathbb{P}(E_2)$, we
divide this event by conditioned on the distance $d(v_{RC},v_1) =i$
then
\begin{equation*}
\begin{aligned}
&\mathbb{P}(E_2)\\ &=P(\hat{v}\neq v_{1}|d(v_{RC},v_1) <
  K/2)\mathbb{P}(d(v_{RC},v_1) <
  K/2)\\ &=\sum_{i=1}^{K/2}P(\hat{v}\neq
  v_{1}|d(v_{RC},v_1)=i)\mathbb{P}(d(v_{RC},v_1) =i),
\end{aligned}
\end{equation*}
where the case $\mathbb{P}(d(v_{RC},v_1) =0)$ is omitted since the
probability $\mathbb{P}(\hat{v}\neq v_{1}|d(v_{RC},v_1)=0)$ becomes
zero.  Then, we first find the probability $\mathbb{P}(\hat{v}\neq
v_{1}|d(v_{RC},v_1)=i)$ when the total budget is $K.$ To do this, let
$X_j$ be the random variable which takes values $+1$ if the answer is
correct and takes $-1$ if the answer is incorrect at $j$-th query
because if the answer is correct then the distance of next queried
node will be deducted by one from the rumor source and vice
versa. Then, for the error event, it should be $\sum_{j=1}^{K/2}X_j <
i$ for all $1\leq j \leq K/2$. Then if $q>1/d$,
\begin{equation*}
\begin{aligned}
\mathbb{P}(\hat{v}\neq v_{1}&|d(v_{RC},v_1)=i)\\ &\leq
\sum_{j=0}^{i-1}\binom{K/2}{j}q^{j}(1-q)^{K/2-j}\\ &=I_{1-q}(K/2-i,i)\\ &=(K/2-i)\binom{K/2}{i-1}\int_{0}^{1-q}t^{K/2-i}(1-t)^{i-1}dt\\ &
\stackrel{(a)}{\leq}
exp\left(-\frac{2((K/2)q-(i-1))^3}{K/2}\right)\\ &\leq exp\left(-2q^3
(K/2)^2\right),\\
\end{aligned}
\end{equation*}
where $(a)$ is due to the Hoeffding bound for the regularized
incomplete beta function $I_{1-q}(K/2-i,i)$ when $q>1/d$. Hence, from
the fact that $\mathbb{P}(d(v_{RC},v_1) \leq K/2)\leq 1$, we obtain
\begin{equation*}
\begin{aligned}
\mathbb{P}(E_2)\leq (K/2)e^{-2q^3 (K/2)^2}.
\end{aligned}
\end{equation*}
Then, combining the probabilities $\text{Pr}(E_1)$ and
$\mathbb{P}(E_2)$, we have the total error bound as
\begin{equation}\label{eqn:error}
\begin{aligned}
\mathbb{P}(\hat{v}\neq v_{1})&=\mathbb{P}(E_1)+\mathbb{P}(E_2)\\ &\leq
c \cdot e^{- K\log (K/2)}+(K/2)e^{-2q^3 (K/2)^2}\\ &\leq( c
+1)(K/2)e^{-2q^3 (K/2)^2}\\ &\stackrel{(a)}{\leq} c_1 e^{-2q^3
  (K/2)\log(K/2)},\\
\end{aligned}
\end{equation}
where $c_1=c+1$ and the inequality $(a)$ is from the fact that
$(K/2)e^{-(K/2)}\leq K/2 = e^{\log (K/2)}$. Then, from this result 
we extend \eqref{eqn:error} for the general $r$. In this case, we also 
use the majority result of answer for the
additional question with noisy probability $q$. 
To obtain this, consider the total number of direction queries is $r\geq1$ and let
$Y^{1}_i(v)$ be the random variable with probability $q$ for the
parent node $i$ takes $+1$ at the $i$-th query and let
$Y^{j}_i(v)$ for other neighbor node $2\leq j\leq d$ with probability
$(1-q)/(d-1)$ takes $+1$ at the $i$-th query. Let $Z_j (v)
=\sum_{i=1}^{r}Y^{j}_i (v)$ and let $\hat{q}:=\mathbb{P}(Z_1 (v) > Z_j
(v),~ 2\leq j \leq d)$ then from the result in \eqref{eqn:error}, we have 
\begin{equation}\label{eqn:err}
\begin{aligned}
\mathbb{P}(\hat{v}\neq v_{1})&\leq ce^{-2\hat{q}^3
  (K/(r+1))\log(K/(r+1))},\\
\end{aligned}
\end{equation}
$c=(8d+1)/d$. To obtain the optimal $r^*$, we consider the following
lemma.

\smallskip
\begin{lemma}
For the redundancy $r$, if $q>1/d$ then
\begin{equation*}
\begin{aligned}
\hat{q}\geq 1- e^{-\frac{r(d-1)}{3d(1-q)}}.
\end{aligned}
\end{equation*}
\label{lem:major}
\end{lemma}
\smallskip
This result is similar version of Lemma~ \ref{lem:majority} which the
proof will be in the next section. If we set $g_d (r,q):= 1-
e^{-\frac{r(d-1)}{3(1-q)}}$ then we complete the proof of Proposition~\ref{prop:inter_prob}. 

\subsection{Proof of Theorem~\ref{thm:interactive}}

To finish the proof, we will obtain
the following lemma for the optimal choice of $r$ from \eqref{eqn:err}
and Lemma~\ref{lem:major}.

\smallskip
\begin{lemma}
For $q>1/d$, the optimal $r^*$ in \eqref{eqn:result1} is given by
\begin{equation}
\begin{aligned}
r^* \simeq \left\lfloor1+\frac{2d(1-q)^2 \log\log
  K}{3(d-1)}\right\rfloor.
\end{aligned}
\end{equation}
\label{lem:redundancy2}
\end{lemma}
\smallskip
By using these two results and \eqref{eqn:error}, we consider the error
probability for a given $r$ as
\begin{equation*}
\begin{aligned}
\mathbb{P}(\hat{v}\neq v_{1})&=\mathbb{P}(E_1)+\mathbb{P}(E_2)\\ &\leq
ce^{-2\hat{q}^3 (K/(r+1))\log(K/(r+1))}\\ &\leq ce^{-2\left(1-
  e^{-\frac{r(d-1)}{3d(1-q)}}\right)^3 (K/(r+1))\log(K/(r+1))}\\ &\leq
ce^{-2\left(1- e^{-(1-q)\log\log K}\right)^3
  (K/(r+1))\log(K/(r+1))}\\ &\stackrel{(a)}{=} ce^{-2\left(1- (\log
  K)^{-(1-q)}\right)^3
  (K/(r+1))\log(K/(r+1))}\\ &\stackrel{(b)}{\leq} ce^{-2e^{q^3} K^2
  \log(K/(r+1))}\\ &\leq ce^{-2e^{q^3} K\log K},\\
\end{aligned}
\end{equation*}
where the equality $(a)$ is from the fact that $1-x \simeq e^{-x}$ for
$x\simeq 0$ and $(b)$ is from the fact that $q>1/d$. Therefore, let
$\delta\geq ce^{-2e^{q^3} K\log K}$ then, by similar approach in \cite{Khim14}, we have if
\begin{equation*}
    \begin{aligned}
     K\geq \frac{c\log(7/\delta)}{q^3\log (\log (7/\delta))},
    \end{aligned}
  \end{equation*}
then $\text{Pr}(\hat{v}= v_{1})\geq 1-\delta$ where $c=(2d-3)/d$. 
Hence, we complete the proof of
Theorem~\ref{thm:interactive}.




























%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "main"
%%%% End:

